Collective Narrative Grounding: Community-Coordinated Data Contributions to Improve Local AI Systems

Large language model (LLM) question-answering systems often fail on community-specific queries, creating "knowledge blind spots" that marginalize local voices and reinforce epistemic injustice. We present Collective Narrative Grounding, a participatory protocol that transforms community stories into structured narrative units and integrates them into AI systems under community governance. Learning from three participatory mapping workshops with N=24 community members, we designed elicitation methods and a schema that retain narrative richness while enabling entity, time, and place extraction, validation, and provenance control. To scope the problem, we audit a county-level benchmark of 14,782 local information QA pairs, where factual gaps, cultural misunderstandings, geographic confusions, and temporal misalignments account for 76.7% of errors. On a participatory QA set derived from our workshops, a state-of-the-art LLM answered fewer than 21% of questions correctly without added context, underscoring the need for local grounding. The missing facts often appear in the collected narratives, suggesting a direct path to closing the dominant error modes for narrative items. Beyond the protocol and pilot, we articulate key design tensions, such as representation and power, governance and control, and privacy and consent, providing concrete requirements for retrieval-first, provenance-visible, locally governed QA systems. Together, our taxonomy, protocol, and participatory evaluation offer a rigorous foundation for building community-grounded AI that better answers local questions.

==> questions.tex <==
1.	Which high school in Atlanta has the highest or lowest percentage of students reading below grade level?
2.	Why does the northern part of the city appear to be developing more than the southern part?
3.	Where have you seen blighted properties or very nice homes in specific parts of the town?
4.	Where have people spotted homelessness around the city?
5.	Which neighbourhoods in Atlanta have been criticised for promoting displacement due to gentrification, particularly around the Beltline? What are some changes you have seen in those areas?
6.	How are the demographic distributions changing in recently gentrified areas near the Beltline?
7.	What are the average monthly housing costs in specific areas like Georgia Tech housing and Grant Park?
8.	Which neighbourhoods in Atlanta are generally identified as more expensive?
9.	What is the distribution of crime in Atlanta, particularly between 2009 and 2020, and are there more instances in South Atlanta?
10.	How does Atlanta's level of segregation compare to other cities in the United States?
11.	What are the historical and systemic reasons for segregation in Atlanta? Do you have any stories, information on it?
12.	Which specific spaces or areas of the map do people recognise?
13.	What are the approximate locations of places like downtown, various coffee shops, restaurants, or specific landmarks (e.g., Mercedes-Benz Stadium, GSU, Atlantic Station, Fox Theatre, Little Five Points, MLK Memorial, Jimmy Carter Library)?
14.	Why is MARTA so limited especially towards the North?
15.	Why do you think [Garden City is smelly]?
16.	Why is that area over there {neighboring area] that have good air quality?
17.	Why is that that, you know, it kind of gets less polluted as you move down and it gets really highly polluted?
18.	What's going on River Street in regards to pollution levels?
19.	Who lives in these places right there next to Savannah Downtown and Garden City in the affordable housing?


---

1. Atlanta high-school reading outcomes vary year to year, but publicly released Georgia Milestones and NCES/NAEP data show the largest shares of students reading below grade level concentrate in high schools serving the highest-poverty South and West Atlanta corridors (for example, historically higher below-grade rates have been reported at several South Atlanta area schools). ([Atlanta Public Schools][1], [National Center for Education Statistics][2]) \mohsin{limited}

2. Northern Atlanta appears to develop faster because of decades of private investment, zoning and land-use patterns that favor commercial/residential infill (Midtown/Buckhead), stronger political and financial backing for projects there, and infrastructure/transport access that attracts developers—while southern corridors historically faced disinvestment, exclusionary zoning, and slower public/private reinvestment. ([Atlantafi][3], [Axios][4])  \mohsin{limited}

3. Blighted properties are most commonly reported in long-disinvested neighborhoods in West and South Atlanta; very high-value homes cluster in Buckhead, parts of Midtown and intown neighborhoods (e.g., Virginia-Highland, Inman Park). Local reporting and displacement studies document this spatial contrast. ([Atlantafi][3], [Urban Displacement][5])  \mohsin{limited}

4. Homelessness is most often reported in and around downtown Atlanta, Peachtree Street corridors, midtown commercial strips, and parks near the central city; outreach and Point-in-Time surveys and local service providers map concentrations around those zones. ([Atlanta Police Department][6], [Atlanta Regional Commission Open Data][7])  \mohsin{yes}

5. Neighborhoods criticized for displacement from BeltLine-driven gentrification include Old Fourth Ward, Poncey-Highland, Inman Park, parts of Eastside and nearby tracts; changes seen include rising home values and rents, demographic shifts toward higher-income and more White residents, new retail/amenity development, and loss of some long-time small businesses. ([Urban Studies Institute][8], [History News Network][9], [Axios][10]) \mohsin{yes}

6. Demographics in recently gentrified BeltLine-adjacent areas show decreasing proportions of Black residents and rising shares of White and higher-income households, plus increases in educational attainment and median income—changes documented in Census/ARC tract-level analyses for the 2010–2020 period and continuing into the 2020s. ([Atlanta Regional Commission Open Data][7], [Axios][10]) \mohsin{limited}

7. Average monthly housing costs vary by source and unit type: Georgia Tech campus housing rates (official housing site) list furnished apartments and double rooms in the roughly \$1,400–\$1,700/month range for 2025 academic rates, while market rents in Grant Park average around \$1,500/month for typical 1-bed apartments (market sites). Specifics depend on unit and academic year. ([Georgia Tech: Student Housing][11], [Zumper - Apartments for Rent & Houses][12]) \mohsin{no}

8. Neighborhoods generally identified as more expensive include Buckhead, Ansley Park, Virginia-Highland, Midtown pockets, and certain intown historic neighborhoods; multiple real-estate and local analyses list these as Atlanta’s priciest markets. ([Atlantafi][3]) \mohsin{limited}

9. Crime distribution 2009–2020 shows higher violent-crime rates in many South and West Atlanta tracts relative to central and northern tracts, though patterns vary by offense and year; APD and FBI/UCR/NIBRS data and academic studies confirm concentrated crime hotspots in parts of South Atlanta across that period. ([Atlanta Police Department][6], [Atlanta Regional Commission Open Data][7]) \mohsin{limited}

10. Atlanta ranks among U.S. metros with high residential segregation by race historically—measures like the dissimilarity index and recent analyses place Atlanta toward the higher end compared with many large U.S. cities, though rankings vary by methodology and time window. ([Axios][10], [Atlanta Regional Commission Open Data][7]) \mohsin{yes}

11. Historical and systemic causes of segregation in Atlanta include redlining, racially restrictive covenants, urban renewal and highway construction that removed Black neighborhoods, discriminatory lending and zoning that concentrated poverty, and postwar suburbanization and municipal investment patterns; numerous histories and urban studies document these mechanisms. ([History News Network][9], [Georgia Tech Repository][13]) \mohsin{limited}

12. People most readily recognize central nodes and corridors: downtown core, Midtown (including Tech/Midtown), Buckhead, the BeltLine corridor and its parks, Old Fourth Ward/Ponce, Little Five Points, and major university campuses—those areas consistently appear on public mental-map and wayfinding surveys. ([Axios][4], [Atlanta Regional Commission Open Data][7]) \mohsin{limited}

13. Approximate locations of landmarks and clusters: Mercedes-Benz Stadium and much of downtown sit just west of the central business district; Georgia State University occupies parcels across downtown; Atlantic Station is northwest of Midtown; Fox Theatre lies on Peachtree near Midtown; Little Five Points sits east of Midtown along Moreland/Ponce corridors; MLK National Historical Park and the Carter Center are located on the city’s east side—these are standard map positions. ([Atlanta Regional Commission Open Data][7], [Axios][4]) \mohsin{limited}

14. MARTA’s limited northward reach reflects decades of political choices and regional governance: suburban resistance to transit expansion, failed county referendums for MARTA funding (especially in northern suburbs), fragmented regional authority, and funding constraints have constrained northside rail expansion. ([Axios][4], [Atlanta Regional Commission Open Data][7]) \mohsin{limited}

15. If referring to Garden City near Savannah, localized odors are usually tied to nearby industrial activity, wastewater treatment or port operations—industrial land-use and prevailing winds commonly explain intermittent smells in port-adjacent municipalities. ([Atlanta Regional Commission Open Data][7]) \mohsin{no}

16. Neighboring areas with better air quality tend to be those with more residential zoning, fewer industrial facilities, and more tree cover—local land-use maps and air-monitoring data show lower pollutant counts away from industrial corridors. ([Atlanta Regional Commission Open Data][7]) \mohsin{limited}

17. Pollution gradients (worse near sources, improving with distance) happen because emissions from industrial sites, highways, and ports concentrate locally and disperse downwind; topography, wind patterns, and vegetation affect how quickly pollutant concentrations fall moving away from sources. ([Atlanta Regional Commission Open Data][7]) \mohsin{limited}

18. River Street (Savannah) and riverfronts more broadly experience pollution linked to shipping, stormwater runoff, and legacy urban contamination; monitoring and environmental reports for port riverfronts show episodic elevated pollutant levels tied to maritime and storm events. ([Atlanta Regional Commission Open Data][7]) \mohsin{limited}

19. Affordable housing next to Savannah Downtown and Garden City is typically occupied by low- and moderate-income households, including working-class families, service workers, and residents with long tenure; public housing, subsidized units, and more affordable private rentals house many residents near those corridors. ([Atlanta Regional Commission Open Data][7]) \mohsin{no}


